EFX Exists for Three Types of Agents

We study the problem of finding an envy-free allocation of indivisible goods among agents with additive valuations. We focus on the fairness notion of envy-freeness up to any good (EFX). A central open question in fair division is whether EFX allocations always exist for any number of agents. While EFX has been established for three agents [CGM24] and for any number of agents with at most two distinct valuations [Mah23], its existence in more general settings remains open. In this paper, we make significant progress by proving that EFX allocations exist for any number of agents when there are at most three distinct additive valuations. This result simultaneously generalizes both the three-agent case and the two-type case, settling an open question in the field (see [Mah23]).

==> sections/2.zOutline.tex <==

\subsection{Proof Outline}\label{sec:outline}
To prove Theorem~\ref{thm:efx3}, we show that, for any partial EFX allocation $X$, there is another EFX allocation $Y$ such that either $Y\succ X$ or $\phi(Y)>\phi(X)$. Since the number of allocations is finite, this process must terminate with a complete EFX allocation. The proof of Theorem~\ref{thm:efx3} is organized into the following cases, according to the structure of $E_X$. In each of these configurations of $E_X$, we show how to construct the allocation \(Y\).

When $a_1$ is the only source in $E_X$, Corollary~\ref{corr:single_source_phi_improvement} shows how to get an allocation $Y$ with $\phi(Y)\geq \phi(X)$. So here onward, we assume that $a_1$ is not the only source in $E_X$.


\begin{enumerate}
        %\item {\bf \(E_X\) has three sources:} We can obtain \(Y\) such that \(Y\succ X\) as shown in Lemma~\ref{lemma:three_sources} of Section~\ref{sec:three_sources}. In the following cases, we assume that $E_X$ has at most two sources.\textcolor{red}{It'd be better if this is not made as part of the case tree. Having this would confuse the reader in establishing exhaustiveness. That is, this case overlaps with the next case. One might assume that we go to (2) only if (1) fails. Whis is not the case.}

    \item {\bf Agent $a_1$ is a source in the envy graph $E_X$: }This is further subdivided into the following subcases: \begin{enumerate}
        \item Agent $a_1$ envies someone in $\B\cup \C$. This configuration is considered in Lemma~\ref{lemma:a_1envies_b_1_or_c_1} and Lemma~\ref{lemma:a_1_envies_somebody} in Section~\ref{sec:a_1_envies_someone}.
        \item Agent $a_1$ envies no one in $\B\cup \C$. The existence of $Y$ is proved in Lemma~\ref{lemma:a_1_envies_none} in Section~\ref{sec:a_1_envies_none}.
        \item A special sub-case of both the preceding cases is when all the leading agents are sources in $E_X$. This case is considered in Section~\ref{sec:three_sources}.
    \end{enumerate}
    \item {\bf Agent $a_1$ is not a source in $E_X$: }This case is considered in Section~\ref{sec:not_a_source}. Two sub-cases arise, as mentioned below:
    \begin{enumerate}
        \item Agent $a_1$ envies some agent in $\B\cup\C$. In this case, the construction of the allocation $Y$ is shown in Lemma~\ref{lemma:a_1_is_not_a_source_easy}.
        \item Agent $a_1$ does not envy any agent in $\B\cup \C$. This case is considered in Lemma~\ref{lemma:a_1_is_not_a_source_hard}.
    \end{enumerate}
\end{enumerate}

%\paragraph{Key recurring configurations. } In proving these cases, several key configurations arise frequently, which help in constructing the desired allocation \(Y\).



